Promoting Counterfactual Robustness through Diversity

Counterfactual explanations shed light on the decisions of black-box models by explaining how an input can be altered to obtain a favourable decision from the model (e.g., when a loan application has been rejected). However, as noted recently, counterfactual explainers may lack robustness in the sense that a minor change in the input can cause a major change in the explanation. This can cause confusion on the user side and open the door for adversarial attacks. In this paper, we study some sources of non-robustness. While there are fundamental reasons for why an explainer that returns a single counterfactual cannot be robust in all instances, we show that some interesting robustness guarantees can be given by reporting multiple rather than a single counterfactual. Unfortunately, the number of counterfactuals that need to be reported for the theoretical guarantees to hold can be prohibitively large. We therefore propose an approximation algorithm that uses a diversity criterion to select a feasible number of most relevant explanations and study its robustness empirically. Our experiments indicate that our method improves the state-of-the-art in generating robust explanations, while maintaining other desirable properties and providing competitive computational performance.

==> table_dice.tex <==
\begin{table*}
    \centering
    % \resizebox{1\columnwidth}{!}{
    \begin{tabular}{ccccccccccc}
        \cline{2-11}&
        \multicolumn{2}{c}{diabetes} &
        \multicolumn{2}{c}{no2} &
        \multicolumn{2}{c}{credit} &
        \multicolumn{2}{c}{spambase} &
        \multicolumn{2}{c}{news} \\
        \cline{2-11}
        & ours & \texttt{DiCE} & ours & \texttt{DiCE} & ours & \texttt{DiCE} & ours & \texttt{DiCE} & ours & \texttt{DiCE}\\
        \hline
        validity & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 48/50 & 50/50 & 50/50 \\ \hline
        $k$-distance  & \textbf{1.18} & 1.90 & \textbf{0.78} & 1.29 & \textbf{0.70} & 1.91 & \textbf{0.71} & 7.83 & \textbf{2.4} & 4.12\\ \hline
        $k$-diversity  & \textbf{1.30} & \textbf{1.30} & \textbf{0.92} & 0.91 & 0.76 & \textbf{2.02} & 0.51 & \textbf{8.62} & \textbf{2.85} & 2.04 \\ \hline
        $\setdist^d_{\Sigma}$  & 0.29 & \textbf{0.28} & \textbf{0.17} & 0.27 & \textbf{0.27} & 0.70 & \textbf{0.57} & 3.73 & \textbf{0.60} & 1.89 \\ \hline
       $\setdist^d_{max}$  & 0.71 & \textbf{0.57} & \textbf{0.43} & 0.56 & \textbf{0.56} & 1.20 & \textbf{0.72} & 7.12 & \textbf{1.53} & 2.90\\ \hline
       Time & \textbf{0.02} & 57.22 & \textbf{0.01} & 116.03 & \textbf{0.13} & 306.42 & \textbf{0.09} & 188.94 & \textbf{0.28} & 351.52  \\ \hline
    \end{tabular}
    % }
    \caption{Comparison between our method and \texttt{DiCE} on $50$ instances. Best results for each metric highlighted in bold.}
    \label{tab:results-dice}
\end{table*}

==> table_single.tex <==
\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccccccccccccc}
        \cline{2-16}&
        \multicolumn{3}{c}{diabetes} &
        \multicolumn{3}{c}{no2} &
        \multicolumn{3}{c}{credit}&
         \multicolumn{3}{c}{spambase} &
        \multicolumn{3}{c}{news}\\
        \cline{2-16}
        & ours & \texttt{DiCE} & \texttt{proto} & ours & \texttt{DiCE} & \texttt{proto} & ours & \texttt{DiCE} & \texttt{proto} & ours & \texttt{DiCE} & \texttt{proto} & ours & \texttt{DiCE} & \texttt{proto}\\
        \hline
        validity & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 50/50 & 48/50 & 50/50 & 50/50& 50/50 & 50/50 \\ \hline
        distance  & 0.97 & 1.92 & \textbf{0.69} & 0.61 & 1.13 & \textbf{0.20} & 0.54 & 1.61 & \textbf{0.39} & 0.66 & 6.63& \textbf{0.20} & 2.09 & 4.13 & \textbf{0.41} \\ \hline
        LOF & \textbf{1.00} & -0.96 & 0.96 & \textbf{1.00} & 0.27 & 0.96 & \textbf{0.52} & -0.48 & 0.44 & \textbf{0.48}& -0.92 & 0.36 & \textbf{1} & -0.8&\textbf{1} \\ \hline
        dist-cfx & 0.15 & 0.14 & \textbf{0.08} & 0.17 & 0.09 & \textbf{0.07} & 0.14 & 0.23 & \textbf{0.10} & \textbf{0.51} &  6.43& 0.76 & \textbf{0.62}&3.00&0.96   \\ \hline
        Time & \textbf{0.01} & 13.23 & 9.23 & \textbf{0.01} & 18.39 & 9.63 & \textbf{0.10} & 50.35 & 9.73 & \textbf{0.05} & 51.61& 11.69 & \textbf{0.22} &69.60&13.44\\ \hline
    \end{tabular}
    }
    \caption{Comparison between our method, \texttt{DiCE} and \texttt{proto} for single counterfactuals on 50 instances. Best results for each metric highlighted in bold.}
    \label{tab:results-single}
\end{table*}
